Open-Vocabulary Temporal Action Detection with Off-the-Shelf Image-Text Features

Detecting actions in untrimmed videos should not be limited to a small, closed set of classes. We present a simple, yet effective strategy for open-vocabulary temporal action detection utilizing pretrained image-text co-embeddings. Despite being trained on static images rather than videos, we show that image-text co-embeddings enable openvocabulary performance competitive with fully-supervised models. We show that the performance can be further improved by ensembling the image-text features with features encoding local motion, like optical flow based features, or other modalities, like audio. In addition, we propose a more reasonable open-vocabulary evaluation setting for the ActivityNet data set, where the category splits are based on similarity rather than random assignment.

==> tmp <==
This is pdfTeX, Version 3.141592653-2.6-1.40.24 (TeX Live 2022/Debian) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./arxiv.tex
LaTeX2e <2022-06-01> patch level 5
L3 programming layer <2022-08-30> (./bmvc2k.cls
Document Class: bmvc2k 2022/07/12 BMVC Proceedings. v0.17
(/usr/share/texlive/texmf-dist/tex/latex/base/article.cls
Document Class: article 2021/10/04 v1.4n Standard LaTeX document class
(/usr/share/texlive/texmf-dist/tex/latex/base/size10.clo))
(/usr/share/texlive/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-def/pdftex.def)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/mathcolor.ltx))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)))
(/usr/share/texlive/texmf-dist/tex/latex/subfigure/subfigure.sty
****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/share/texlive/texmf-dist/tex/latex/subfigure/subfigure.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/share/texlive/texmf-dist/tex/latex/eso-pic/eso-pic.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texlive/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/share/texlive/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/share/texlive/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/share/texlive/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/share/texlive/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/share/texlive/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/share/texlive/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/share/texlive/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/share/texlive/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texlive/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/share/texlive/texmf-dist/tex/generic/gettitlestring/gettitlestring.sty
(/usr/share/texlive/texmf-dist/tex/latex/kvoptions/kvoptions.sty)))
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texlive/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/share/texlive/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty)
(/usr/share/texlive/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/share/texlive/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/share/texlive/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/share/texlive/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texlive/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/share/texlive/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty
(/usr/share/texlive/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty)))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texlive/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/share/texlive/texmf-dist/tex/generic/iftex/ifvtex.sty))
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/mathptmx.sty)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/helvet.sty)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/courier.sty)
(./bmvc2k_natbib.sty) Finished loading BMVC2K)
(/usr/share/texlive/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/t1phv.fd)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/ot1ztmcm.fd)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/omlztmcm.fd)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/omsztmcm.fd)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/omxztmcm.fd)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/t1ptm.fd)
(/usr/share/texlive/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./arxiv.aux

LaTeX Warning: Label `tab:anet_proposals_supp' multiply defined.

) (/usr/share/texlive/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texlive/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex

Underfull \hbox (badness 10000) in paragraph at lines 53--53


Underfull \hbox (badness 1009) in paragraph at lines 53--53
[][]\T1/phv/b/n/17.28 Open-Vocabulary Tem-po-ral Ac-tion

Overfull \hbox (35.26196pt too wide) in paragraph at lines 53--53
[][][][] 
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/ts1ptm.fd)
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021{/var/lib/texmf/fonts/map/pdftex/updmap/pd
ftex.map}
BMVC cite {Jia, Yang, Xia, Chen, Parekh, Pham, Le, Sung, Li, and Duerig} 2021
BMVC cite {Pham, Dai, Ghiasi, Liu, Yu, Luong, Tan, and Le} 2021
BMVC cite {Gu, Lin, Kuo, and Cui} 2021
BMVC cite {Zareian, Rosa, Hu, and Chang} 2021
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Luo, Ji, Zhong, Chen, Lei, Duan, and Li} 2021
BMVC cite {Wang, Xing, and Liu} 2021
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022 [1]
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Jia, Yang, Xia, Chen, Parekh, Pham, Le, Sung, Li, and Duerig} 2021
BMVC cite {Pham, Dai, Ghiasi, Liu, Yu, Luong, Tan, and Le} 2021
Overfull \hbox (6.69502pt too wide) in paragraph at lines 78--79
[]\T1/ptm/m/n/10 A sur-vey of fea-tures to com-ple-ment image-text co-embedding
 fea-tures for class-agnostic
BMVC cite {Deng, Dong, Socher, Li, Li, and Fei-Fei} 2009
BMVC cite {Sun, Shrivastava, Singh, and Gupta} 2017
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Jia, Yang, Xia, Chen, Parekh, Pham, Le, Sung, Li, and Duerig} 2021
BMVC cite {Pham, Dai, Ghiasi, Liu, Yu, Luong, Tan, and Le} 2021
BMVC cite {Bansal, Sikka, Sharma, Chellappa, and Divakaran} 2018
BMVC cite {Rahman, Khan, and Barnes} 2020
BMVC cite {Zhu, Wang, and Saligrama} 2020
BMVC cite {Li, Yao, Zhang, Wang, Kanhere, and Zhang} 2019
BMVC cite {Zareian, Rosa, Hu, and Chang} 2021
BMVC cite {Gu, Lin, Kuo, and Cui} 2021
BMVC cite {Zareian, Rosa, Hu, and Chang} 2021
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Luo, Ji, Zhong, Chen, Lei, Duan, and Li} 2021
BMVC cite {Wang, Xing, and Liu} 2021
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Luo, Ji, Zhong, Chen, Lei, Duan, and Li} 2021
BMVC cite {Wang, Xing, and Liu} 2021
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022 [2]
BMVC cite {Islam and Radke} 2020
BMVC cite {Narayan, Cholakkal, Hayat, Khan, Yang, and Shao} 2021
BMVC cite {Wang, Xiong, Lin, and Van\protect \unhbox \voidb@x \protect \penalty
 \@M \ {}Gool} 2017
BMVC cite {Chao, Vijayanarasimhan, Seybold, Ross, Deng, and Sukthankar} 2018
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Shou, Chan, Zareian, Miyazawa, and Chang} 2017
BMVC cite {Zeng, Huang, Tan, Rong, Zhao, Huang, and Gan} 2019
BMVC cite {Zhao, Xiong, Wang, Wu, Tang, and Lin} 2020{}
BMVC cite {Lin, Liu, Li, Ding, and Wen} 2019
BMVC cite {Wang, Zhang, Zheng, and Pan} 2022
BMVC cite {Xu, Zhao, Rojas, Thabet, and Ghanem} 2020
BMVC cite {Zhang, Wu, and Li} 2022
BMVC cite {Xiong, Wang, Wang, Zhang, Song, Li, Lin, Qiao, Gool, and Tang} 2016
BMVC cite {Wentao\protect \unhbox \voidb@x \protect \penalty \@M \ {}Bao} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Wentao\protect \unhbox \voidb@x \protect \penalty \@M \ {}Bao} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Chao, Vijayanarasimhan, Seybold, Ross, Deng, and Sukthankar} 2018
BMVC cite {Lin, Liu, Li, Ding, and Wen} 2019
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Shou, Chan, Zareian, Miyazawa, and Chang} 2017
BMVC cite {Xu, Zhao, Rojas, Thabet, and Ghanem} 2020
BMVC cite {Zeng, Huang, Tan, Rong, Zhao, Huang, and Gan} 2019
BMVC cite {Zhao, Xiong, Wang, Wu, Tang, and Lin} 2020{} [3 <./architecture_v5.p
df>] BMVC cite {Gu, Lin, Kuo, and Cui} 2021
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Zareian, Rosa, Hu, and Chang} 2021
BMVC cite {Fabian Caba\protect \unhbox \voidb@x \protect \penalty \@M \ {}Heilb
ron and Niebles} 2015
BMVC cite {Idrees, Zamir, Jiang, Gorban, Laptev, Sukthankar, and Shah} 2016
BMVC cite {Alwassel, Caba\protect \unhbox \voidb@x \protect \penalty \@M \ {}He
ilbron, Escorcia, and Ghanem} 2018 [4]
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Luo, Ji, Zhong, Chen, Lei, Duan, and Li} 2021
BMVC cite {Wang, Xing, and Liu} 2021 BMVC cite {Carreira and Zisserman} 2017
BMVC cite {Hershey, Chaudhuri, Ellis, Gemmeke, Jansen, Moore, Plakal, Platt, Sa
urous, Seybold, Slaney, Weiss, and Wilson} 2017 BMVC cite {Tensorflow} 2020
BMVC cite {Fabian Caba\protect \unhbox \voidb@x \protect \penalty \@M \ {}Heilb
ron and Niebles} 2015
BMVC cite {Idrees, Zamir, Jiang, Gorban, Laptev, Sukthankar, and Shah} 2016
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022 [5]
BMVC cite {Carion, Massa, Synnaeve, Usunier, Kirillov, and Zagoruyko} 2020
BMVC cite {Newell, Yang, and Deng} 2016 BMVC cite {Ba, Kiros, and Hinton} 2016
BMVC cite {Duan, Bai, Xie, Qi, Huang, and Tian} 2019
BMVC cite {Huang, Rathod, Sun, Zhu, Korattikara, Fathi, Fischer, Wojna, Song, G
uadarrama, et\protect \unhbox \voidb@x \protect \penalty \@M \ {}al.} 2017
BMVC cite {Alwassel, Giancola, and Ghanem} 2021
BMVC cite {Carreira and Zisserman} 2017
BMVC cite {Kay, Carreira, Simonyan, Zhang, Hillier, Vijayanarasimhan, Viola, Gr
een, Back, Natsev, Suleyman, and Zisserman} 2017
BMVC cite {Arnab, Dehghani, Heigold, Sun, Lu{£}i{¢}, and Schmid} 2021
BMVC cite {Hershey, Chaudhuri, Ellis, Gemmeke, Jansen, Moore, Plakal, Platt, Sa
urous, Seybold, Slaney, Weiss, and Wilson} 2017
BMVC cite {Gemmeke, Ellis, Freedman, Jansen, Lawrence, Moore, Plakal, and Ritte
r} 2017 BMVC cite {Tensorflow} 2020
BMVC cite {Jia, Yang, Xia, Chen, Parekh, Pham, Le, Sung, Li, and Duerig} 2021
BMVC cite {Pham, Dai, Ghiasi, Liu, Yu, Luong, Tan, and Le} 2021
BMVC cite {Sun, Shrivastava, Singh, and Gupta} 2017
BMVC cite {Nagrani, Yang, Arnab, Jansen, Schmid, and Sun} 2021{}
BMVC cite {Gemmeke, Ellis, Freedman, Jansen, Lawrence, Moore, Plakal, and Ritte
r} 2017 BMVC cite {Nagrani, Yang, Arnab, Jansen, Schmid, and Sun} 2021{}
BMVC cite {Kay, Carreira, Simonyan, Zhang, Hillier, Vijayanarasimhan, Viola, Gr
een, Back, Natsev, Suleyman, and Zisserman} 2017
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Nagrani, Seo, Seybold, Hauth, Manen, Sun, and Schmid} 2022
BMVC cite {Luo, Ji, Zhong, Chen, Lei, Duan, and Li} 2021
BMVC cite {Wang, Xing, and Liu} 2021
BMVC cite {Arnab, Dehghani, Heigold, Sun, Lu{£}i{¢}, and Schmid} 2021
BMVC cite {Nagrani, Yang, Arnab, Jansen, Schmid, and Sun} 2021{}
BMVC cite {Xiong, Wang, Wang, Zhang, Song, Li, Lin, Qiao, Gool, and Tang} 2016
[6]
BMVC cite {Xiong, Wang, Wang, Zhang, Song, Li, Lin, Qiao, Gool, and Tang} 2016
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Jia, Yang, Xia, Chen, Parekh, Pham, Le, Sung, Li, and Duerig} 2021
BMVC cite {Pham, Dai, Ghiasi, Liu, Yu, Luong, Tan, and Le} 2021
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin
, Clark, Krueger, and Sutskever} 2021
BMVC cite {Jia, Yang, Xia, Chen, Parekh, Pham, Le, Sung, Li, and Duerig} 2021
BMVC cite {Pham, Dai, Ghiasi, Liu, Yu, Luong, Tan, and Le} 2021
BMVC cite {Carreira and Zisserman} 2017
BMVC cite {Carreira and Zisserman} 2017 BMVC cite {Tensorflow} 2020
BMVC cite {Hershey, Chaudhuri, Ellis, Gemmeke, Jansen, Moore, Plakal, Platt, Sa
urous, Seybold, Slaney, Weiss, and Wilson} 2017
BMVC cite {Arnab, Dehghani, Heigold, Sun, Lu{£}i{¢}, and Schmid} 2021
BMVC cite {Nagrani, Yang, Arnab, Jansen, Schmid, and Sun} 2021{}
BMVC cite {Nagrani, Yang, Arnab, Jansen, Schmid, and Sun} 2021{}
Underfull \hbox (badness 1292) in paragraph at lines 365--365
\T1/ptm/m/n/10 de-tec-tor ar-chi-tec-tures with dif-fer-ent in-put fea-tures. O
n Ac-tiv-i-tyNet, mAP@Avg is
[7] BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
Overfull \hbox (0.6012pt too wide) in paragraph at lines 423--425
 [][] 
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
Underfull \vbox (badness 10000) has occurred while \output is active [8]
[9] BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Zeng, Huang, Tan, Rong, Zhao, Huang, and Gan} 2019
BMVC cite {Su, Xu, Sheng, and Ouyang} 2020
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Lin, Xu, Luo, Wang, Tai, Wang, Li, Huang, and Fu} 2021
BMVC cite {Zhang, Wu, and Li} 2022
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Su, Xu, Sheng, and Ouyang} 2020
BMVC cite {Zeng, Huang, Tan, Rong, Zhao, Huang, and Gan} 2019
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Lin, Xu, Luo, Wang, Tai, Wang, Li, Huang, and Fu} 2021
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Zhang, Wu, and Li} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022 [10] (./arxiv.bbl
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/t1pcr.fd) [11] [12] [13]
Underfull \hbox (badness 4582) in paragraph at lines 307--311
[]\T1/ptm/m/n/10 Tensorflow.  Mod-els/research/audioset/yamnet at mas-ter \TS1/
ptm/m/n/10 · \T1/ptm/m/n/10 ten-sor-flow/models,

Underfull \hbox (badness 10000) in paragraph at lines 353--361
\T1/pcr/m/n/10 content _ CVPR _ 2020 / html / Xu _ G-[]TAD _ Sub-[]Graph _ Loca
lization _
[14]
Underfull \hbox (badness 10000) in paragraph at lines 401--409
[][]$\T1/pcr/m/n/10 https : / / openaccess . thecvf . com / content _ CVPR _ 20
20 / html / Zhu _

Underfull \hbox (badness 10000) in paragraph at lines 401--409
\T1/pcr/m/n/10 Dont _ Even _ Look _ Once _ Synthesizing _ Features _ for _ Zero
-[]Shot _
) [15] BMVC cite {Duan, Bai, Xie, Qi, Huang, and Tian} 2019
BMVC cite {Carion, Massa, Synnaeve, Usunier, Kirillov, and Zagoruyko} 2020
BMVC cite {Duan, Bai, Xie, Qi, Huang, and Tian} 2019
BMVC cite {Carion, Massa, Synnaeve, Usunier, Kirillov, and Zagoruyko} 2020
BMVC cite {Newell, Yang, and Deng} 2016
BMVC cite {Ronneberger, Fischer, and Brox} 2015 [16 <./detection_architectures.
pdf>]
BMVC cite {Carion, Massa, Synnaeve, Usunier, Kirillov, and Zagoruyko} 2020
BMVC cite {Chao, Vijayanarasimhan, Seybold, Ross, Deng, and Sukthankar} 2018
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Duan, Bai, Xie, Qi, Huang, and Tian} 2019
BMVC cite {Duan, Bai, Xie, Qi, Huang, and Tian} 2019
BMVC cite {Duan, Bai, Xie, Qi, Huang, and Tian} 2019 [17 <./rfp.png>]
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Arnab, Dehghani, Heigold, Sun, Lu{£}i{¢}, and Schmid} 2021
BMVC cite {Nagrani, Yang, Arnab, Jansen, Schmid, and Sun} 2021{} [18]
Underfull \vbox (badness 10000) has occurred while \output is active [19 <./thu
mos_map.png>] BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022 [20]
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Ju, Han, Zheng, Zhang, and Xie} 2022
BMVC cite {Shou, Chan, Zareian, Miyazawa, and Chang} 2017
BMVC cite {Xu, Das, and Saenko} 2017
BMVC cite {Zhao, Xiong, Wang, Wu, Tang, and Lin} 2020{}
BMVC cite {Chao, Vijayanarasimhan, Seybold, Ross, Deng, and Sukthankar} 2018
BMVC cite {Zeng, Huang, Tan, Rong, Zhao, Huang, and Gan} 2019
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Xiong, Wang, Wang, Zhang, Song, Li, Lin, Qiao, Gool, and Tang} 2016
BMVC cite {Zeng, Huang, Tan, Rong, Zhao, Huang, and Gan} 2019
BMVC cite {Zhao, Xie, Ju, Zhang, Wang, and Tian} 2020{}
BMVC cite {Yang, Peng, Zhang, Fu, and Han} 2020
BMVC cite {Lin, Liu, Li, Ding, and Wen} 2019
BMVC cite {Xu, Zhao, Rojas, Thabet, and Ghanem} 2020
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Liu, Wang, Hu, Tang, Bai, and Bai} 2021
BMVC cite {Xiong, Wang, Wang, Zhang, Song, Li, Lin, Qiao, Gool, and Tang} 2016
BMVC cite {Xiong, Wang, Wang, Zhang, Song, Li, Lin, Qiao, Gool, and Tang} 2016
BMVC cite {Nagrani, Yang, Arnab, Jansen, Schmid, and Sun} 2021{}
BMVC cite {Stroud, Ross, Sun, Deng, Sukthankar, and Schmid} 2020
Underfull \vbox (badness 6461) has occurred while \output is active [21]

LaTeX Warning: Float too large for page by 4.72133pt on input line 1330.


Overfull \hbox (0.68796pt too wide) in paragraph at lines 1837--1840
 [][] 
[22] [23] [24] [25] [26] [27] [28] [29] [30] [31] [32] [33] (./arxiv.aux)

LaTeX Warning: There were multiply-defined labels.

 )
(see the transcript file for additional information){/usr/share/texlive/texmf-d
ist/fonts/enc/dvips/base/8r.enc}</usr/share/texlive/texmf-dist/fonts/type1/publ
ic/amsfonts/cm/cmex10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/ams
fonts/cm/cmmi10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/
cm/cmr10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy
10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/symbols/msbm1
0.pfb></usr/share/texlive/texmf-dist/fonts/type1/urw/courier/ucrr8a.pfb></usr/s
hare/texlive/texmf-dist/fonts/type1/urw/helvetic/uhvb8a.pfb></usr/share/texlive
/texmf-dist/fonts/type1/urw/helvetic/uhvr8a.pfb></usr/share/texlive/texmf-dist/
fonts/type1/urw/times/utmb8a.pfb></usr/share/texlive/texmf-dist/fonts/type1/urw
/times/utmbi8a.pfb></usr/share/texlive/texmf-dist/fonts/type1/urw/times/utmr8a.
pfb></usr/share/texlive/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/share
/texlive/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on arxiv.pdf (33 pages, 481224 bytes).
Transcript written on arxiv.log.

